Deep Reward Supervisions for Tuning Text-to-Image Diffusion Models

Optimizing a text-to-image diffusion model with a given reward function is an important but underexplored research area. In this study, we propose Deep Reward Tuning (DRTune), an algorithm that directly supervises the final output image of a text-to-image diffusion model and back-propagates through the iterative sampling process to the input noise. We find that training earlier steps in the sampling process is crucial for low-level rewards, and deep supervision can be achieved efficiently and effectively by stopping the gradient of the denoising network input. DRTune is extensively evaluated on various reward models. It consistently outperforms other algorithms, particularly for low-level control signals, where all shallow supervision methods fail. Additionally, we fine-tune Stable Diffusion XL 1.0 (SDXL 1.0) model via DRTune to optimize Human Preference Score v2.1, resulting in the Favorable Diffusion XL 1.0 (FDXL 1.0) model. FDXL 1.0 significantly enhances image quality compared to SDXL 1.0 and reaches comparable quality compared with Midjourney v5.2.

==> tables/main_table.tex <==
\begin{table}
  \centering
  \resizebox{0.9\textwidth}{!}{
  \begin{tabular}{lcccc}
    \toprule
    Method & HPS v2.1$\uparrow$ & PickScore$\uparrow$ & Aesthetic Score$\uparrow$ & Symmetry$\downarrow$ \\
    \midrule
    ReFL-10~\cite{xu2023imagereward} & 39.18 & 0.2488 & 9.585 & 0.7512 \\
    ReFL-20~\cite{xu2023imagereward} & 39.43 & 0.2491 & 9.911 & 0.7328 \\ 
    DRaFT-LV~\cite{clark2023directly} & 39.02 & 0.2477 & 9.615 & 0.7648 \\
    DRaFT-10~\cite{clark2023directly} & 37.62 & 0.2456 & 8.317 & 0.7250 \\
    AlignProp~\cite{prabhudesai2023aligning} & 34.04 & 0.2297 & 6.627 & 0.7840 \\
    \midrule
    DRTune (outs) & \textbf{39.68} & \textbf{0.2492} & \textbf{9.914} & \textbf{0.3716} \\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparison with baseline methods. We report the average reward computed on prompts from the HPS v2~\cite{wu2023humanv2} benchmark.}
  \label{tab:main_result}
\end{table}

==> tables/train_step_sampling.tex <==
\begin{table}
  \label{tab:train_sampling}
  \centering
  \resizebox{0.35\textwidth}{!}{
  \begin{tabular}{lccc}
    \toprule
    Reward & HPS v2.1$\uparrow$  & Symmetry$\downarrow$ \\
    \midrule
    last 5 steps & 38.44 & 0.6922 \\
    random 5 steps & 38.04 & \textbf{0.4958} \\
    weighted random 5 steps & \textbf{38.90} & 0.5976 \\
    \bottomrule
  \end{tabular}
  }
  \caption{Comparison between different methods for sampling training steps.}
\end{table}
